Scheduling of Wireless Edge Networks for Feedback-Based Interactive Applications

Interactive applications with automated feedback will largely influence the design of future networked infrastructures. In such applications, status information about an environment of interest is captured and forwarded to a compute node, which analyzes the information and generates a feedback message. Timely processing and forwarding must ensure the feedback information to be still applicable; thus, the quality-of-service parameter for such applications is the end-to-end latency over the entire loop. By modelling the communication of a feedback loop as a two-hop network, we address the problem of allocating network resources in order to minimize the delay violation probability (DVP), i.e. the probability of the end-to-end latency exceeding a target value. We investigate the influence of the network queue states along the network path on the performance of semi-static and dynamic scheduling policies. The former determine the schedule prior to the transmission of the packet, while the latter benefit from feedback on the queue states as time evolves and reallocate time slots depending on the queue's evolution. The performance of the proposed policies is evaluated for variations in several system parameters and comparison baselines. Results show that the proposed semi-static policy achieves close-to-optimal DVP and the dynamic policy outperforms the state-of-the-art algorithms.

==> sections/bkp-4-offline-scheduling.tex <==
\sz{spacing will be adjusted in the final draft}
\note{\section{Static Scheduling Policies}\label{sec:offline-scheduling}
%The derivation of exact DVP values is not tractable as it requires the calculation of the probability of union of $w$ events that are not mutually disjoint.
In this section, we derive an upper bound for DVP, referred to as DVPUB, and formulate an upper bound minimization problem, which is then used to compute the proposed static policies. 

Using \emph{union bound} for DVP in~\eqref{eq:exact-dvp2q}, we obtain DVPUB, given by
\begin{IEEEeqnarray}{rCl}
	\IEEEeqnarraymulticol{3}{l}{
		\text{DVPUB}(w,y,x_1,x_2) = 
	}\nonumber\\* \quad
	&&\P\left\{\S^2(1+w) \! < \! y + x_1 + x_2\right\} + \nonumber\\
	&& \sum_{u=1}^{1+w} \P\left\{\S^2(1+w-u) + \S^1(u-1) < y + x_1\right\} \nonumber\\
	&& = \P\left\{\S^2(1+w) \! \leq \! y + x_1 + x_2 - 1\right\} + \nonumber\\
	%&& \P\left\{\S_2(w) \! \leq \! y + x_1 - 1\right\} + \nonumber\\
	&& \sum_{u=1}^{1+w} \P\left\{\S^2(1+w-u) + \S^1(u-1) %\nonumber\\ &&
	 \leq\! y + x_1 -1\right\}.\label{eq:dvpub}
\end{IEEEeqnarray}

%DVPUB is the sum of CDF of the cumulative service of the second server $\S_2$ and the CDF of the sum of the cumulative services of servers $\S_1,\S_2$.
Applying Eq.~\eqref{eq:cumulative-service} to Eq.~\eqref{eq:dvpub}, the DVPUB resulting from the allocation of $\mathbf{n}^2 = \{n^1_1, \dots, n^1_w\}$ slots at the second transmitter and $\mathbf{n}^2=N-\mathbf{n}^1$ slots at the first one is given by
\begin{IEEEeqnarray}{rCl}
	\IEEEeqnarraymulticol{3}{l}{
		\text{DVPUB}(w,y,x_1,x_2,\mathbf{n}^2) =%= \P\{\W(1) > w\}
	}\nonumber\\* \quad
	%	&=&\P\left\{\S_2(1+w) \! < \! y + x_1 + x_2\right\} + \nonumber\\
	%	&& \sum_{u=1}^{1+w} \P\left\{\S_2(1+w-u) + \S_1(u) < y + x_1\right\}\nonumber\\
	&&\quad\sum_{x=0}^{y+x_1+x_2-1}\P\left\{\sum_{i=0}^{w} s_i^2\left(n_i^2\right) = x\right\}\nonumber\\
	%&&+\sum_{y=0}^{y+x_1-1}\P\left\{\B\left(\sum_{i=0}^{w-1} n_i^2,1-p_e\right) = y\right\}\nonumber\\
	&&\quad+\sum_{u=1}^{1+w} \sum_{z=0}^{y+x_1-1} \P\left\{\sum_{j=0}^{w-u} s_j^2\left(n_j^2\right)+\sum_{k=0}^{u-2}s_k^1 \left( n_k^1\right) = z \right\} \nonumber%\\
\end{IEEEeqnarray}
\begin{IEEEeqnarray}{rCl}
	\IEEEeqnarraymulticol{3}{l}{}\nonumber\\* \quad
	&\symtext{(1)}{=}&\quad \sum_{x=0}^{y+x_1+x_2-1} \left(\frac{1}{p_e}-1\right)^x {\sum_{i=0}^{w}n_i^2\choose x} p_e^{\sum_{i=0}^{w}n_i^2}\notag\\
	%&&+ \sum_{y=0}^{y+x_1-1} \left(\frac{1}{p_e}-1\right)^x {\sum_{i=0}^{w-1}n_i^2\choose y} p_e^{\sum_{i=0}^{w-1}n_i^2}\notag\\
	&&\quad+\sum_{u=1}^{1+w} \sum_{z=0}^{y+x_1-1} \left(\frac{1}{p_e}-1\right)^z  p_e^{\sum_{j=0}^{w-u}n_j^2-\sum_{k=0}^{u-2}n_k^2+(u-1)N}\nonumber\\
	&&\quad{\sum_{j=0}^{w-u}n_i^2-\sum_{k=0}^{u-2}n_j^2+(u-1)N\choose z}.\nonumber\\*\label{eq:dvpub-w-server}
\end{IEEEeqnarray}
 In step (1), we used the fact that $S^i(k)$ is distributed as a Binomial r.v. as shown in Eq.~\eqref{eq:cumulative-service}. 
We are interested in minimizing the DVPUB to find static scheduling policies.
However, from Eq.~\eqref{eq:dvpub-w-server}, we observe that DVPUB consists in the sum of Binomial distributions, which are not convex.
\sz{exemplary plot of non convexity when same n is used is for the entire vector}
Therefore, following a similar approach as in~\cite{champati2018transient} a looser convex bound, referred to as Wireless Transient Bound (WTB), is obtained
by applying the \emph{Chernoff bound} to Eq.~\eqref{eq:dvpub}.
\begin{IEEEeqnarray}{rCl}
	\IEEEeqnarraymulticol{3}{l}{
		\text{WTB}(w,y,x_1,x_2) =
	}\nonumber\\
	&&\quad\min_{s>0} \E\left[e^{-s \, \S^2(1+w)}\right] e^{s\,(y + x_1 +x_2 -1)} + \nonumber\\
	%&& \E\left[e^{-s \, \S_2(w)}\right] e^{s\,(y + x_1 -1)} + \nonumber\\
	&&\quad\sum_{u=1}^{1+w} \E\left[e^{-s \left[ \S^1(u-1)+\S^2(1+w-u)\right]}\right] e^{s\,(y + x_1 -1)},\label{eq:wtb}
\end{IEEEeqnarray}

Following the approach in~\cite{champati2018transient}, the calculation of WTB for a wireless transmitter is obtained by computing the Mellin transform of the cumulative service of Eq.~\eqref{eq:cumulative-service}
\begin{align}
	\mathbb{E}\left[e^{-s \, \S(m,\mathbf{n})}\right] &= \mathbb{E}\left[e^{-s \, \sum_{i=0}^{-1+\sum_{j=0}^{m-1} n_j} b_i}\right] \nonumber\\
	&=\mathbb{E}\left[\left(e^{-s \, b_i}\right)^{\sum_{i=0}^{m-1} n_i}\right]\nonumber\\
	&= \left[(1-p_e)e^{-s}+p_e\right]^{\sum_{i=0}^{m-1} n_i},\nonumber\\*\label{eq:mellin-dynamic-server} 
\end{align}
where $b_i$ indicates the i.i.d. Bernoulli random variables of each transmission outcome.

Finally, combining Eq.~\eqref{eq:wtb} and~\eqref{eq:mellin-dynamic-server}, we obtain
\begin{IEEEeqnarray}{rCl}
	\IEEEeqnarraymulticol{3}{l}{
		\text{WTB}(w,y,x_1,x_2,\mathbf{n}^2) =
	}\nonumber\\* \quad
	%&=&\min_{s>0} \E\left[e^{-s \, \S_2(1+w)}\right] e^{s\,(y + x_1 +x_2 -1)} + \nonumber\\
	%&& \sum_{u=1}^{1+w} \E\left[e^{-s \left[ \S_1(u)+\S_2(1+w-u)\right]}\right] e^{s\,(y + x_1 -1)} \nonumber\\
	%&=& \min_{s>0} \mathbb{E}\left[e^{-s \, \sum_{i=0}^{-1+\sum_{j=0}^{w} n_j^2} b_i}\right] e^{s\,(y + x_1 +x_2 -1)} +\nonumber\\
	%&& \sum_{u=1}^{1+w} \E\left[e^{-s  \left[\sum_{i=0}^{-1+\sum_{j=0}^{u-1-1} N-n_j^2+\sum_{j=0}^{w-u} n_j^2} b_i\right]}\right] e^{s\,(y + x_1 -1)} \nonumber\\
	&&\quad \min_{s>0} \left[(1-p_e) e^{-s}+p_e \right]^{\sum_{i=0}^{w} n_i^2} e^{s\,(y + x_1 +x_2 -1)} + \nonumber\\
	&&\quad \sum_{u=1}^{1+w} \left[(1-p_e) e^{-s}+p_e\right]^{(u-1)N-\sum_{j=0}^{u-2} n_j^2+\sum_{i=0}^{w-u} n_i^2} \nonumber\\
	&&\quad e^{s\,(y + x_1 -1)}.\label{eq:wtb-w-server}
\end{IEEEeqnarray}

Given the initial queue backlogs $\mathbf{q}_0 = \left\lbrace x_1,x_2\right\rbrace$, we aim to solve the upper bound minimization problem below
% the static scheduling policy, denoted by $\pi^\star_1\left(\mathbf{q}_0\right)$, that minimizes Eq. \eqref{eq:wtb-w-server}, is given by
\begin{equation}
\pi^\star_1\left(\mathbf{q}_0\right) \, = \argmin_{\mathbf{n}^2 \in \left\{1,\dots,N-1\right\}}\text{WTB}(w,y,x_1,x_2,\mathbf{n}^2) .\label{eq:wtb-opt}
\end{equation}

As shown by Theorem~\ref{th1}, a solution to the problem of Eq.~\eqref{eq:wtb-opt} can be efficiently derived when the domain of the optimization variable $\mathbf{n}^2$ is continuous.
This can be achieved by solving
\begin{equation}
\widetilde{\pi}^\star_S\left(\mathbf{q_0}\right) \, = \argmin_{\mathbf{n}^2 \in \left[1,N-1\right]^w}\text{WTB}(w,y,x_1,x_2,\mathbf{n}^2) ,\label{eq:wtb-opt-relaxed}
\end{equation}
then, by converting $\widetilde{\pi}^\star_S$ to the integer domain to find a feasible solution to Eq.~\eqref{eq:opt-static}, thus obtaining the scheduling policy $\hat{\pi}^\star_S$.

\begin{theorem}\label{th1}
	The optimization problem in~\eqref{eq:wtb-opt-relaxed} is convex.
\end{theorem}
\begin{proof}
The proof is given in Appendix~\ref{app:wtb2q-convexity}.
\end{proof}

Thanks to Theorem~\ref{th1}, well-known convex optimization algorithms can be used, such as the subgradient or interior-point, which provide scalability for an increasing number of slots $N$ and frames within the deadline $w$.
In this work, the relaxed problem is solved using the nonlinear programming solver \emph{fmincon} available in Matlab\texttrademark~employing the sequential quadratic programming (SQP) algorithm.
Once $\widetilde{\pi}^\star_S$ is found, a conversion to the integer domain is needed in order to determine $\hat{\pi}^\star_S$.
Although the optimal selection of an integer solution would require the exploration of the entire problem's domain, heuristic methods can be applied to find a solution in the neighbourhood of $\widetilde{\pi}^\star_S$.
To this end, we investigate different neighbour search methods in order to achieve near-optimal performances.

The simplest way to derive $\hat{\pi}^*_{S}$ is to round each frame allocation of $\widetilde{\pi}^\star_S$ to its closest integer value.
We refer to this method as WTB-R.
Alternatively, the heuristic policy can be found in the neighbourhood of the continuous solution.
For each frame allocation $n^1_i \in \widetilde{\pi}^\star_S$, two integer values are derived applying the floor and ceiling functions.
A reduced search space is constructed computing all the combinations of the integer values for each frame until the deadline, which leads to a total of $2^w$ combinations.
As final step, Eq.~\eqref{eq:dvpub-w-server} and \eqref{eq:wtb-w-server} are used to evaluate each combination and identify the best one.
The static policies corresponding to the evaluation of Eq.~\eqref{eq:dvpub-w-server} and \eqref{eq:wtb-w-server} over this search space are referred to as WTB-D and WTB-W, respectively.

The performances of the different heuristics have been evaluated via extensive simulations of a broad range of values for each system parameter, i.e. for $x_1, x_2$~$\in$ ~$\left\{0,1,2\right\}$, $w$~$\in$~$\left\{2,3,4,5,6\right\}$, $N$~$\in$~$\left\{2,3,4,5\right\}$, and $p_e$~$\in$~$\left\{0.2,0.33,0.4,0.5\right\}$.
For performance comparison, two additional schedulers have been evaluated, eDVPUB and eWTB, which exhaustively explore the problem's domain to find the policies that respectively achieve the minimum values of DVPUB, cf. Eq.~\eqref{eq:dvpub-w-server}, and WTB, cf. Eq.~\eqref{eq:wtb-w-server}.
Furthermore, the performance of each scheduler is compared with the performance of the policy that achieves the minimum DVP.
This optimal policy is found by exploring the DVP of all possible policies via simulations.
%Thus, the policies obtained by eDVPUB and eWTB are computed evaluating $N^w$ times .

Fig.~\ref{fig:1-boxplot-offline} shows the performance of the proposed static schedulers by computing, for each scheduler and system configuration, the percentage of existing policies that achieve higher DVP.
% This calculat
% with respect to the optimal policy that achieves the minimum DVP.
% For each parameter, the performance of each policy is expressed using the ranking the performance
As expected, the exhaustive search methods eWTB and eDVPUB achieve the best results, with eDVPUB finding, in the large majority of cases, the top $10\%$ static policies.
The performance gap between eWTB and eDVPUB is introduced by the Chernoff bound in Eq.~\eqref{eq:mellin-dynamic-server}.
These methods, however, are not efficient as they require the exhaustive exploration of the entire problem domain.
The heuristic methods WTB-R/W/D can be used to efficiently find static policies for a broad range of parameters.
The low complex WTB-R achieves the worst performance.
Interestingly, WTB-W and WTB-D achieve similar performances of the exhaustive methods, with WTB-W achieving better performances.
This can be explained by the fact that, in WTB-D, Eq.~\eqref{eq:wtb-w-server} is used to solve the relaxed problem, while Eq.~\eqref{eq:dvpub-w-server} to find the integer solution.
%This discrepancy results in reduced performance.
}

\begin{figure}[!t]
	\centering
	\includegraphics{./results/fig_boxplot_ws_x1s_x2s_pes_Ns_algs_aggr_percentages.pdf}
	\caption{Performance of the proposed static schedulers for different system parameters. For each scheduler, the percentage of existing policies that achieve higher DVP is evaluated.}
	\label{fig:1-boxplot-offline}
\end{figure}
